A Probabilistic-Logic based Commonsense Representation Framework for Modelling Inferences with Multiple Antecedents and Varying Likelihoods

Commonsense knowledge-graphs (CKGs) are important resources towards building machines that can 'reason' on text or environmental inputs and make inferences beyond perception. While current CKGs encode world knowledge for a large number of concepts and have been effectively utilized for incorporating commonsense in neural models, they primarily encode declarative or single-condition inferential knowledge and assume all conceptual beliefs to have the same likelihood. Further, these CKGs utilize a limited set of relations shared across concepts and lack a coherent knowledge organization structure resulting in redundancies as well as sparsity across the larger knowledge graph. Consequently, today's CKGs, while useful for a first level of reasoning, do not adequately capture deeper human-level commonsense inferences which can be more nuanced and influenced by multiple contextual or situational factors. Accordingly, in this work, we study how commonsense knowledge can be better represented by -- (i) utilizing a probabilistic logic representation scheme to model composite inferential knowledge and represent conceptual beliefs with varying likelihoods and (ii) incorporating a hierarchical conceptual ontology to identify salient concept-relevant relations and organize beliefs at different conceptual levels. Our resulting knowledge representation framework can encode a wider variety of world knowledge and represent beliefs flexibly using grounded concepts as well as free-text phrases. As a result, the framework can be utilized as both a traditional free-text knowledge graph and a grounded logic-based inference system more suitable for neuro-symbolic applications. We describe how we extend the PrimeNet knowledge base with our framework through crowd-sourcing and expert-annotation, and demonstrate its application for more interpretable passage-based semantic parsing and question answering.

==> approach_old.tex <==
\iffalse
\begin{table}[t]
\small
\setlength\tabcolsep{1.4pt}
\begin{tabular}{|wc{0.16\columnwidth}|wl{0.49\columnwidth}|wl{0.37\columnwidth}|}%{|l|l|l|} %r
\hline
\rowcolor{Gray}
Term & Description & Examples\\
\hline
Predicate & \makecell{A relation (e.g. isa, causes) \\ or attribute (e.g. size, color)} & \makecell{isa, shape\\ related\_to, color..} \\
\hline
Constant & \makecell{A term that is grounded \\ and fixed (e.g. numbers,\\ text-phrases and symbols \\ with lower-case first letter)} & \makecell{`X eats Y', -23, \\ person, `Bob', x} \\
\hline
Variable & \makecell{An ungrounded term that \\ takes value during inference. \\Starts with an upper-case char \\} & \makecell{X, Y, Event, \\Bob, Person} \\
\hline
%\toprule
Atom & \makecell{A predicate with n arguments \\ Syntax: pred(arg0,arg1..)} & \makecell{isa(person,physical) \\ has\_part(car,wheel,4)} \\
\hline
%\midrule
\makecell{Prob.\\Fact} & \makecell{A declarative belief with \\  a given base likelihood (if  \\ unspecified assumed to be 1)} & \makecell{0.5::can(x,buy,car).\\0.98::has(person,face).\\isa(person,physical).} \\

\hline
\makecell{Prob.\\ Clause\\/ Rule} & \makecell{An inferential belief where\\  a head atom `h' is inferred \\ with a base clause likelihood \\  $P_c$ from computation of body \\ (or antecedent) set of atoms \\ (denoted by `b') as follows:\\ $P(h)=P_c \times \prod{P(b)}$} & \makecell{0.9:: head:-a1,(a2;a3).\\ 0.6::can(X,move):-\\has(X,leg).\\0.95::can(X,buy,Y):-\\has(X,Z),(value(Z)\\$>=$value(Y)).} \\
\hline
%\makecell{Logical \\operators} & \makecell{And is denoted by `,' \\ Or is denoted by `;' \\ Not is denoted by `$\backslash+$' \\ Clause is denoted by `:-'} & \makecell{can(X,move):-\\(has(X,wheel);\\has(X,leg)),\\$\backslash+$(state(X,stuck)).} \\

%\hline

Model & \makecell{Corresponds to a set of facts \\ and rules representing a \\world `model' on which \\inferences can be performed} & \makecell{0.5::can(item,move).\\0.9::can(X,move):-\\(has(X,wheel);\\has(X,leg)). \\} \\
\hline

Query & \makecell{An atomic query to infer from \\  a given world likelihood of a  \\ fact (e.g. can(human,move)?) \\or valid constants for variables \\ (e.g. can(X,move)?) } & \makecell{can(human,move)? \\$=>$ 0.9 \\ can(X,move)?\\$=>$ X=item (0.5); \\X= human(0.9) ..} \\
\hline
\end{tabular}\caption{Terms and ProbLog syntax relevant to our work's discussion.}\label{table:approach:primer}
\end{table}
\fi

We aim to design a knowledge representation and reasoning scheme that can effectively model inferential knowledge comprising multiple antecedents and represent beliefs with varying likelihoods. Additionally, our target representation scheme should allow for the knowledge to be utilized as both a free-text knowledge-graph and a grounded semantic inference system. As mentioned previously, we will utilize a probabilistic logic programming approach to model such knowledge and perform inferences. Specifically, we utilize the ProbLog language \cite{Raedt2007ProbLogAP,de2015probabilistic} for our work given its well-developed framework \cite{Fierens2014InferenceAL,dries2015problog2}, and its extensions for relational learning and neuro-symbolic processing \cite{manhaeve2018deepproblog}, which are both relevant to our future directions on designing learning-based approaches for acquiring such knowledge. %our work.%  well as its integration of learning mechanisms and available extensions such as DeepProblog \cite{manhaeve2018deepproblog} for neuro-symbolic processing, which are both relevant to future directions of our work. 

\subsection{Probabilistic logic programming primer / syntax}
Probabilistic logic programming extends traditional logic programming \cite{lloyd2012foundations} (as in Prolog) with probabilities attached to facts and clauses to model uncertainties. Table \ref{table:approach:primer} lists probabilistic logic programming terminology and ProbLog syntax relevant to our work's discussion. An example representation of the natural language belief \textit{`X can move with base likelihood 0.9 if X has a leg or a wheel and X is not in a stuck state'} in logical form is ``\texttt{0.9::can(X,move):- (has(X,leg); has(X,wheel)), not(state(X,stuck)).}" Here `;' denotes `logical or' and `,' denotes `logical and'. For a more comprehensive overview of probabilistic logic programming, we refer the reader to \cite{de2015probabilistic}. %The equivalent nested free-text tuple representation is ``\textit{ ((`X', can, `move'), if, (((`X', has, `leg'), or, (`X', has, `wheel')), and, (not,(`X', state, `stuck'))))}".

%Further, as per ProbLog, we denote logical operators `and' with `,' `OR' with `;', `NOT' with `$backslash$


\begin{table}[t]
\small
\setlength\tabcolsep{1.4pt}
\begin{tabular}{|wc{0.16\columnwidth}|wl{0.49\columnwidth}|wl{0.37\columnwidth}|}%{|l|l|l|} %r
\hline
\rowcolor{Gray}
Term & Description & Examples\\
\hline
Predicate & \makecell{A relation (e.g. isa, causes) \\ or attribute (e.g. size, color)} & \makecell{isa, shape\\ related\_to, color..} \\
\hline
Constant & \makecell{A term that is grounded \\ and fixed (e.g. numbers,\\ text-phrases and symbols \\ with lower-case first letter)} & \makecell{`X eats Y', -23, \\ person, `Bob', x} \\
\hline
Variable & \makecell{An ungrounded term that \\ takes value during inference. \\Starts with an upper-case char \\} & \makecell{X, Y, Event, \\Bob, Person} \\
\hline
%\toprule
Atom & \makecell{A predicate with n arguments \\ Syntax: pred(arg0,arg1..)} & \makecell{isa(person,physical) \\ has\_part(car,wheel,4)} \\
\hline
%\midrule
\makecell{Prob.\\Fact} & \makecell{A declarative belief with \\  a given base likelihood (if  \\ unspecified assumed to be 1)} & \makecell{0.5::can(x,buy,car).\\0.98::has(person,face).\\isa(person,physical).} \\

\hline
\makecell{Prob.\\ Clause\\/ Rule} & \makecell{An inferential belief where\\  a head atom `h' is inferred \\ with a base clause likelihood \\  $P_c$ from computation of body \\ (or antecedent) set of atoms \\ (denoted by `b') as follows:\\ $P(h)=P_c \times \prod{P(b)}$} & \makecell{0.9:: head:-a1,(a2;a3).\\ 0.6::can(X,move):-\\has(X,leg).\\0.95::can(X,buy,Y):-\\has(X,Z),(value(Z)\\$>=$value(Y)).} \\
\hline
%\makecell{Logical \\operators} & \makecell{And is denoted by `,' \\ Or is denoted by `;' \\ Not is denoted by `$\backslash+$' \\ Clause is denoted by `:-'} & \makecell{can(X,move):-\\(has(X,wheel);\\has(X,leg)),\\$\backslash+$(state(X,stuck)).} \\

%\hline

Model & \makecell{Corresponds to a set of facts \\ and rules representing a \\world `model' on which \\inferences can be performed} & \makecell{0.5::can(item,move).\\0.9::can(X,move):-\\(has(X,wheel);\\has(X,leg)). \\} \\
\hline

Query & \makecell{An atomic query to infer from \\  a given world likelihood of a  \\ fact (e.g. can(human,move)?) \\or valid constants for variables \\ (e.g. can(X,move)?) } & \makecell{can(human,move)? \\$=>$ 0.9 \\ can(X,move)?\\$=>$ X=item (0.5); \\X= human(0.9) ..} \\
\hline
%Noisy-or & \makecell{isa; can;\\ related\_to} & \makecell{isa(X,Z):-\\isa(X,Y),isa(X,Z)} \\
%\hline
%Root & \makecell{isa; can;\\ related\_to} & \makecell{isa(X,Z):-\\isa(X,Y),isa(X,Z)} \\
%\hline
%Root & \makecell{isa; can;\\ related\_to} & \makecell{isa(X,Z):-\\isa(X,Y),isa(X,Z)} \\
%\rowcolor{LightCyan}
%\hline 
\end{tabular}\caption{Terms and ProbLog syntax relevant to our work's discussion.}\label{table:approach:primer}
\end{table}
\iffalse
\begin{itemize}
    \item \textbf{Atom}: An atom refers to a predicate of arity n, having n arguments that can each be a variable (ungrounded elements that start with an upper-case can be referpredicate(constant, variable2) e.g. has(human, brain) ; has(X,brain)
    \item \textbf{Fact}: single atom 
    \item \textbf{Clause}:
    \item \textbf{Probabilistic fact}
    \item \textbf{Probabilistic rule}
    \item \textbf{Annotated disjunctions}
    \item \textbf{Querying}
    \item \textbf{Representing base beliefs that update with evidence Noisy OR when multiple beliefs updating base likelihood}
    %\item \textbf{List logic}
    
\end{itemize}
\fi


%\scriptsize
\iffalse
\begin{tabular}{|l|c|c|} %r
\hline
- & Knowledge \\
%\toprule
Model & \multicolumn{2}{|c|}{ImageNet(V1)} \\
%\hline
%- & Top1 & Top5   \\
\hline
%\midrule
Knowledge & isa(x,x1) & isa(x,x2)   \\
\hline
Query & 58.54   \\
\hline
Inference & 56.62 & 67.88 \\ 
%\rowcolor{LightCyan}
\hline 
\end{tabular}



    
Stuff
i) Atom: predicate(constant, constant2)
ii) Fact -- single atom
iii) Clause -- 
iii) Model
i) Probabilistic fact
ii) Probabilistic rule (variables and computation)
iii) Querying (Backward inferences)
iv) Multiple base + noisy-or
v) List logic
For more, we refer the reader to Prob 
Specifically, we use the ProbLog language which has a well-developed inference engine and also encompasses
\fi
%KT-NET 


\subsection{Knowledge representation and reasoning scheme}
To illustrate our knowledge representation and reasoning scheme, we make use of the format as in table \ref{}
\textbf{General fact and rule representations.}
predicate(N,S,T,X)

-- How it helps in interepretablity (show an example where interpertablity trace is produced with knowledge source)

-- How text phrases utilized when conceptually grounded knowledge is not available (this is equivalent to current KB scheme)




\textbf{Show example with noisy or for updating beliefs}

\textbf{Ontological arrangement with cross-inheritance}. Concepts vs names vs instances (provided by


\textbf{Declaritive knowledge lookup.}
Querying by concept (constant) vs by concept name

\textbf{Concept knowledge -- Verb schemas (event representations)} (e.g. what happens next)

\textbf{Situational knowledge} (e.g. selectional restriction?)

\textbf{Physical laws and numerical reasoning} (e.g. gas law, likely object) any others?) -- something is likely to be 

\textbf{Affordance knowledge} (e.g. selectional restriction -- X more

\textbf{Higher-order concept inference} (e.g. vegetarian; afford)

\subsection{Base conceptual ontology and predicates}
0. Distinct from WordNet as here our focus is not lexical coverage but for identification of salient predicates and organizing beliefs 
1. Utilize semantic roles from VerbNet
2. Base conceptual ontology from KT paper -- directed acyclic graph 
3. Predicates were identified by us based on ontological nodes
4. Table on ontology and salient predicates 
5. Upon this framework, new knowledge can be simply added by providing new facts and rules

\begin{table}[h]
\small
\setlength\tabcolsep{3pt}
\begin{tabular}{|wl{0.05\columnwidth}|wl{0.9\columnwidth}|}%{|p{1\columnwidth}|}%{|l|} %r
%Knowledge
\rowcolor{Gray}
\hline
%\multicolumn{8}{|c|}{Sets}
\multicolumn{2}{|l|}{Knowledge} \\ 
\hline
F1 & uses(X,terminal)\\
F2 & can(X,program) \\
%Query
\rowcolor{Gray}
\hline 
\multicolumn{2}{|l|}{Example queries} \\ 
\hline
%\makecell{Q1: isa(X,person)\\Q2: isa(X, person), can(X, program)} \\
Q1 & isa(X,person)?\\ 
Q2 & isa(X, person), can(X, program)? \\
%Inference
\rowcolor{Gray}
\hline 
\multicolumn{2}{|l|}{Inferences} \\ 
\hline
\multirow{2}{*}{I1} &  1.0: isa(programmer, person), 1.0: isa(lawyer, person)  \\& 1.0: isa(student, person), 1.0: isa(ada, person)..  \\ 
\hline
\multirow{2}{*}{I2} &  1.0: isa(programmer, person), 1.0: isa(lawyer, person)  \\& 1.0: isa(student, person), 1.0: isa(ada, person)..  \\ 
%\makecell{uses(X,terminal)\\can(X,program)} \\
\hline

\end{tabular}\label{table:approach1}
\end{table}


\subsection{Utilization as grounded inference system and free-text knowledge graph}
Sample templates table 1
Table 2 with original form and mapped forms
%\subsection
%\subsection{Knowledge annotation methods}
%\textbf{Crowdsourcing and manual annotation}

%\textbf{Implementation details}

%1. Knowledge representation and reasoning scheme
- Probabilistic Logic primer
- Preliminearies: Predicates, constants and variables, types
- Describe ProbLog -- facts and rules -- derivation of inferences
-- Why we use -- simple to be learnable by future methods , and draws on problog / neuro-symbolic approaches and abductive learning .. -- limited in quantifiers
-- Neodavidsonian representations; Utilize semantic-roles for events rather than predicates to better model
-- Discourse relations not yet captured
-- Limitations 


%2. Knowledge collection (How knowledge is collected)
-- Ontology and predicates (and reduced subset of WordNet -- our ontology can be linked to wordnet)
-- Crowdsourcing method
-- Domain-expert annotation

%3. Knowledge applications and inference mechanisms
-- Given shallow tuples, the task is to convert 

%a. 

%2. Conceptual ontology and predicates
-- 
-- predicates are arranged
-- salient set of predicates; full set is displayed in appendix and also
-- usage in few-shot 
-- Make a table with predicate; description; Parent Type; Example; ConceptNet / Atomic2020relation (mark None/- to indicate not present)

%3. Knowledge inference
- Describe Problog
- Example rules and types
-- Make a table with rule; description; Example usage
-- Verb schemas - Neodavidsonian representation
-- Physics laws
-- 

%Direct knowledge-lookup

%Scenario based inference -- provided conditions, perform query

%4. Encoding knowledge
%%-- Rule-based
%%-- Crowdsourcing
%%-- Existing resources

